Data-Driven Abstraction-Based Control Synthesis

This paper studies formal synthesis of controllers for continuous-space systems with unknown dynamics to satisfy requirements expressed as linear temporal logic formulas. Formal abstraction-based synthesis schemes rely on a precise mathematical model of the system to build a finite abstract model, which is then used to design a controller. The abstraction-based schemes are not applicable when the dynamics of the system are unknown. We propose a data-driven approach that computes the growth bound of the system using a finite number of trajectories. The growth bound together with the sampled trajectories are then used to construct the abstraction and synthesise a controller. Our approach casts the computation of the growth bound as a robust convex optimisation program (RCP). Since the unknown dynamics appear in the optimisation, we formulate a scenario convex program (SCP) corresponding to the RCP using a finite number of sampled trajectories. We establish a sample complexity result that gives a lower bound for the number of sampled trajectories to guarantee the correctness of the growth bound computed from the SCP with a given confidence. We also provide a sample complexity result for the satisfaction of the specification on the system in closed loop with the designed controller for a given confidence. Our results are founded on estimating a bound on the Lipschitz constant of the system and provide guarantees on satisfaction of both finite and infinite-horizon specifications. We show that our data-driven approach can be readily used as a model-free abstraction refinement scheme by modifying the formulation of the growth bound and providing similar sample complexity results. The performance of our approach is shown on three case studies.

==> table1.tex <==
% !TEX root = main.tex

\begin{table*}[t]
	\large
	\centering
	\caption{Implementation results for the case studies.
		\textmd{Number of sample trajectories $N$ for each pair $(\xh,\uh)$, run times in minutes for synthesising controllers, and the size of the winning region $|\mathcal V|$. We have used a fixed discretisation in Algorithm~\ref{alg:main_abstraction} both without and in presence of disturbance (OOT stands for out of time, we fixed the bound 10 hours).
			%Dimension of case studies both for state space ($|X|$) and input space ($|U|$), 
			% For local ABCD, the reported numbers correspond to the maximum value among all of the agents.
		}
		\label{tab:runtimes}
	}
	
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{0.7em} % for the horizontal padding
	%\resizebox{1\columnwidth}{!}{
	\begin{tabular}{l|cc|c|ccc}%|ccc}
		\toprule
		Case-study&\multicolumn{2}{c|}{Dimension}& Disturbance& 
		\multicolumn{3}{c}{Fixed dicretisation}\\%&\multicolumn{3}{c}{Iterative Refinement}\\
		
		&$X$&$U$&&$N$& time (min)&$|\mathcal V|$\\%&$N$&$t$&$|\text{Win}|$\\
		\midrule
		
		%$\multirow{2}{*}{\rotatebox{0}{Path planning}}&$3$&$2$&&&&&&\\
		\multirow{2}{*}{\rotatebox{0}{Path planning}} &\multirow{2}{*}{\rotatebox{0}{$3$}}&\multirow{2}{*}{\rotatebox{0}{$2$}}&$\text{Without Disturbance}$& $50$ & $190$  & $106266$\\%& $3258$&$1364$&106540 \\
		&&&$\text{with Disturbance}$& $600$ & $\text{OOT}$  & $\text{OOT}$\\%& $4424$&2306&$143146$ \\
		\midrule
		\multirow{2}{*}{\rotatebox{0}{DC-DC boost converter}} &\multirow{2}{*}{\rotatebox{0}{$2$}}&\multirow{2}{*}{\rotatebox{0}{$1$}}&$\text{Without Disturbance}$& $82$&$3$  & $44722$\\%&$???$&$????$&$183820$\\
		&&&$\text{with Disturbance}$& $105$&$4$  & $41865$\\%&$???$&$???$&$???$\\		
		%\midrule
		
		%\multirow{1}{*}{\rotatebox{0}{Power grid}} & $4$&$1$ & $???$&$???$  & $ 4858056$&$???$&$???$&$8714304$\\
		
		\bottomrule
	\end{tabular}%}
\end{table*}
